Expressive Score-Based Priors for Distribution Matching with Geometry-Preserving Regularization

Distribution matching (DM) is a versatile domain-invariant representation learning technique that has been applied to tasks such as fair classification, domain adaptation, and domain translation. Non-parametric DM methods struggle with scalability and adversarial DM approaches suffer from instability and mode collapse. While likelihood-based methods are a promising alternative, they often impose unnecessary biases through fixed priors or require explicit density models (e.g., flows) that can be challenging to train. We address this limitation by introducing a novel approach to training likelihood-based DM using expressive score-based prior distributions. Our key insight is that gradient-based DM training only requires the prior's score function -- not its density -- allowing us to train the prior via denoising score matching. This approach eliminates biases from fixed priors (e.g., in VAEs), enabling more effective use of geometry-preserving regularization, while avoiding the challenge of learning an explicit prior density model (e.g., a flow-based prior). Our method also demonstrates better stability and computational efficiency compared to other diffusion-based priors (e.g., LSGM). Furthermore, experiments demonstrate superior performance across multiple tasks, establishing our score-based method as a stable and effective approach to distribution matching. Source code available at https://github.com/inouye-lab/SAUB.

==> inouye-macros.tex <==
\ProvidesPackage{macros}
% \newtheorem{theorem}{Theorem}
% \newtheorem{lemma}[theorem]{Lemma}
% \newtheorem{corollary}[theorem]{Corollary}
% \newtheorem{proposition}{Proposition}
% \theoremstyle{definition}
% \newtheorem{definition}{Definition}
% \theoremstyle{definition}
% \newtheorem{intuition}{Intuition}
% \theoremstyle{definition}
% \newtheorem{observation}{Observation}
% \theoremstyle{definition}
% \newtheorem{hypothesis}{Hypothesis}
% \theoremstyle{definition}
% \newtheorem{remark}{Remark}
% \theoremstyle{definition}
% \newtheorem{conjecture}{Conjecture}
% \theoremstyle{definition}
% \newtheorem{question}{Question}

% \renewcommand{\definitionautorefname}{Def.}
% \renewcommand{\propositionautorefname}{Proposition}
% \renewcommand{\remarkautorefname}{Remark}
% \renewcommand{\lemmaautorefname}{Lemma}
% \renewcommand{\corollaryautorefname}{Corollary}
\newcommand{\algorithmautorefname}{Alg.}
\renewcommand{\equationautorefname}{Eqn.}
\renewcommand{\figureautorefname}{Fig.}
\renewcommand{\sectionautorefname}{Section}

% \renewcommand{\algorithmicrequire}{\textbf{Input:}}
% \renewcommand{\algorithmicensure}{\textbf{Output:}}


\DeclareMathOperator*{\argmin}{arg\,min\,}
\DeclareMathOperator*{\argmax}{arg\,max\,}

\newcommand{\prob}{p}
\newcommand{\expect}{\mathbb{E}}
\newcommand{\given}{\,|\,}
\newcommand{\dgiven}{\,\|\,}

\newcommand{\Z}{\ensuremath{\mathbb{Z}}}
\newcommand{\Zp}{\ensuremath{\Z_{+}}}
\newcommand{\Zn}{\ensuremath{\Z_{-}}}
\newcommand{\R}{\ensuremath{\mathbb{R}}}
\newcommand{\Rp}{\ensuremath{\R_{+}}}
\newcommand{\Rn}{\ensuremath{\R_{-}}}

\newcommand{\loss}{\mathcal{L}}

%% Parameters
\newcommand{\nobs}{n}
\newcommand{\ninst}{\nobs}
\newcommand{\nvar}{d}
\newcommand{\ndim}{\nvar}
\newcommand{\nlayer}{k}
\newcommand{\nlayers}{\nlayer}
\newcommand{\depth}{\nlayers}
\newcommand{\nleaves}{J}
\newcommand{\nclasses}{k}

%% Indices
\newcommand{\oldij}{\ij}
\newcommand{\oldit}{\it}
\newcommand{\ii}{i}
\renewcommand{\ij}{j}
\newcommand{\is}{s}
\renewcommand{\it}{t}
\newcommand{\il}{\ell}
\newcommand{\ik}{k}

%% Data/variable macros
\newcommand{\oldu}{\u}

\newcommand{\x}{x}
\newcommand{\xvec}{\bm{\x}}
\newcommand{\xmat}{X}
\newcommand{\xset}{\mathcal{\xmat}}
\newcommand{\y}{y}
\newcommand{\yvec}{\bm{\y}}
\newcommand{\ymat}{Y}
\newcommand{\yset}{\mathcal{\ymat}}
\newcommand{\z}{z}
\newcommand{\zvec}{\bm{\z}}
\newcommand{\zmat}{Z}
\newcommand{\zset}{\mathcal{\zmat}}

\renewcommand{\r}{r}
\newcommand{\rvec}{\bm{\r}}
\newcommand{\rmat}{R}
\newcommand{\rset}{\mathcal{\rmat}}


\newcommand{\xhat}{\widehat{x}}
\newcommand{\xhatvec}{\widehat{\bm{x}}}
\newcommand{\xhatmat}{\widehat{X}}
\newcommand{\yhat}{\widehat{y}}
\newcommand{\yhatvec}{\widehat{\bm{y}}}
\newcommand{\yhatmat}{\widehat{Y}}
\newcommand{\zhat}{\widehat{z}}
\newcommand{\zhatvec}{\widehat{\bm{z}}}
\newcommand{\zhatmat}{\widehat{Z}}
\newcommand{\uhat}{\widehat{u}}
\newcommand{\uhatvec}{\widehat{\bm{u}}}
\newcommand{\uhatmat}{\widehat{U}}
\newcommand{\vhat}{\widehat{v}}
\newcommand{\vhatvec}{\widehat{\bm{v}}}
\newcommand{\vhatmat}{\widehat{V}}

% Unit vectors
\renewcommand{\u}{u}
\newcommand{\uvec}{\bm{\u}}
\newcommand{\umat}{U}
\newcommand{\uset}{\mathcal{\umat}}
\renewcommand{\v}{v}
\newcommand{\vvec}{\bm{\v}}
\newcommand{\vmat}{V}
\newcommand{\vset}{\mathcal{\vmat}}
\renewcommand{\prob}{p}
\newcommand{\probvec}{\bm{\prob}}
\newcommand{\probmat}{P}
\newcommand{\probset}{\mathcal{\probmat}}

\newcommand{\w}{w}
\newcommand{\wvec}{\bm{\w}}
\newcommand{\wmat}{W}
\newcommand{\wset}{\mathcal{\wmat}}

\newcommand{\cset}{\mathcal{C}}
\newcommand{\basedist}{\pi}
\newcommand{\meanvec}{\bm{\mu}}
\newcommand{\normal}{\mathcal{N}}
\newcommand{\I}{\mathbf{I}}

% Distributions
\newcommand{\p}{\mathbb{P}}
\newcommand{\q}{{\hat{p}}}
\newcommand{\qset}{{\mathcal{M}}}

% Target of q distribution
\newcommand{\tq}{\pi}
\newcommand{\tqvec}{\bm{\tq}}
\newcommand{\tqmat}{\Pi}
\newcommand{\tqset}{\mathcal{\tqmat}}

\newcommand{\projp}{\tilde{q}}
\newcommand{\projpvec}{\tilde{\bm{q}}}
\newcommand{\projpmat}{\hat{Q}}
\newcommand{\projpset}{\hat{\mathcal{Q}}}


%% Functions for KL divergence
\newcommand{\KL}{\textnormal{KL}}
\newcommand{\diag}{\text{diag}}
\newcommand{\T}{\text{T}} % Sufficient statistic
\newcommand{\supp}{\textnormal{supp}}
\newcommand{\diff}{\textrm{d}} % Differential
\newcommand{\E}{\mathbb{E}}
\newcommand{\FE}{\mathcal{F}} % Free energy
\newcommand{\wass}{\mathcal{W}}
\newcommand{\growass}{\textnormal{GW}}
\newcommand{\gromon}{\textnormal{GM}}
\newcommand{\Lip}{\textnormal{Lip}}

%% Functions from previous IVT "paper"
\newcommand{\deepfunc}{\Psi}
\newcommand{\deepfuncinv}{\widetilde{\deepfunc}}
\newcommand{\inputspace}{\mathcal{I}}
\newcommand{\outputspace}{\R}
\newcommand{\neuronfunc}{\omega}
\newcommand{\neuronfuncvec}{\Omega}
\newcommand{\orthogonal}{Q}
\newcommand{\univdist}{q}
\newcommand{\cdf}{F}
\newcommand{\cdfvec}{\bm{F}}
\newcommand{\nreduced}{k}
\newcommand{\mutual}{\mathcal{I}}
\newcommand{\entropy}{\mathcal{H}}
\newcommand{\kldiv}{D_{\text{KL}}}
\newcommand{\niter}{m}
\newcommand{\nbin}{b}
\newcommand{\ncomp}{k}

\newcommand\independent{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}

%% Macros for maximum entropy notation
\newcommand{\reg}{R}
\newcommand{\f}{f}
\newcommand{\fvec}{\bm{f}}
\newcommand{\fset}{\mathcal{F}}
\newcommand{\g}{g}
\newcommand{\gvec}{\bm{g}}
\newcommand{\gset}{\mathcal{G}}

%% Macros from deep presentation
\newcommand{\JSD}{\textnormal{JSD}}
\newcommand{\G}{G}
\newcommand{\D}{D}
\newcommand{\infernet}{\D}
\newcommand{\leaf}{\mathcal{L}}
\newcommand{\invset}{\mathcal{I}}

%% Macro for displaying equation inside of tabular environment
\newcommand{\arrayreset}{\hspace{-0.5em}}
\newcommand{\tabeqn}[1]{\( \arrayreset \begin{array}[t]{l} \displaystyle #1 \end{array} \)}

%% Macros for distribution distance
\newcommand{\dist}{d}
\newcommand{\struct}{\mathcal{S}}

\newcommand{\one}{\mathbbm{1}}

\renewcommand{\dist}{d}
\renewcommand{\loss}{\mathcal{L}}

\newcommand{\Hcross}{H_{\textnormal{C}}}
\newcommand{\hl}[1]{{\color{red} #1}}

\newcommand{\pset}{\mathcal{P}}
\newcommand{\dset}{\mathcal{D}}
\newcommand{\tagcomment}[1]{&\text{(#1)}}
\newcommand{\Ra}{R}
\newcommand{\Rb}{\tilde{R}}

%
\newcommand{\Iwe}{I\xspace}
\newcommand{\IWe}{I\xspace}
\newcommand{\myour}{my\xspace}
\newcommand{\MyOur}{My\xspace}

%%%%%%%%%%% New
\newcommand{\onehalf}{{\textstyle \frac{1}{2}}}
\newcommand{\mix}{\textnormal{mix}}
\newcommand{\PXone}{P_{X_1}}
\newcommand{\PXtwo}{P_{X_2}}
\newcommand{\PXmix}{P_{X_{\mix}}}
\newcommand{\PZone}{P_{Z_1}}
\newcommand{\PZtwo}{P_{Z_2}}
\newcommand{\PZmix}{P_{Z_{\mix}}}
\newcommand{\elbo}{\textnormal{ELBO}}
\newcommand{\pcl}{\textnormal{PCL}}
\newcommand{\vpcl}{\textnormal{VPCL}}

\renewcommand{\d}{d}
\DeclareMathOperator{\GJSD}{GJSD}
\newcommand{\OT}{\textnormal{OT}}

% Jim macros
\newcommand{\ourloss}{\mathcal{L}_\mathrm{SAUB}}
% \renewcommand{\baselinestretch}{0.95} % Slightly reduce line spacing
% \setlength{\textfloatsep}{8pt} % Adjust space between text and figures
% \setlength{\intextsep}{8pt} % Space between text and inline floats
% \setlength{\abovecaptionskip}{6pt} % Space above caption
% \setlength{\belowcaptionskip}{0pt} % Space below caption
% \usepackage{enumitem}
% \setlist{nosep} % Removes extra spacing
% \vspace{-2mm} % To reduce space between text and equations
% \usepackage[compact]{titlesec} % Reduces default spacing
% \setlength{\intextsep}{16pt}   % Space above and below wrapfigure
% \setlength{\columnsep}{10pt}  % Space between text and wrapfigure
% % \setlength{\textheight}{\dimexpr\textheight+0mm\relax} % Add 3mm to text height
% \usepackage{placeins}
% \setlength{\topsep}{8pt}       % Space above the proposition
% \setlength{\partopsep}{0pt}    % Space for nested environments

% % \usepackage[top=1in, bottom=0.95in, left=1in, right=1in]{geometry
% \captionsetup{width=\dimexpr\textwidth-2em\relax}



